Bayesian filtering for nonlinear stochastic systems using holonomic gradient method with integral transform

This paper proposes a symbolic-numeric Bayesian filtering method for a class of discrete-time nonlinear stochastic systems to achieve high accuracy with a relatively small online computational cost. The proposed method is based on the holonomic gradient method (HGM), which is a symbolic-numeric method to evaluate integrals efficiently depending on several parameters. By approximating the posterior probability density function (PDF) of the state as a Gaussian PDF, the update process of its mean and variance can be formulated as evaluations of several integrals that exactly take into account the nonlinearity of the system dynamics. An integral transform is used to evaluate these integrals more efficiently using the HGM than our previous method. Further, a numerical example is provided to demonstrate the efficiency of the proposed method compared to other existing methods.

==> latexmkrc <==
#!/usr/bin/perl

# How to Use ############################################################ 
# 
# For Japanese articles:
#       * Uncomment "Use platex" and comment out "Use pdflatex" in 1.
#       * Uncomment 3.
#       * Set 4. to "3"
#
# For English articles:
#       * Uncomment "Use pdflatex" and comment out "Use platex" in 1.
#       * Comment out 3.
#       * Set 4. to "1"
# 
#########################################################################

#--------------------------------------------------#
# 1. Compile Command Setting
#--------------------------------------------------#

##### Use platex (for Japanese articles) #####
#$latex = 'platex %O -src-specials -shell-escape -file-line-error -halt-on-error -interaction=nonstopmode -synctex=1 -kanji=utf8 %S';

##### Use pdflatex (for English articles) #####
$latex = 'pdflatex %O -src-specials -shell-escape -file-line-error -halt-on-error -interaction=nonstopmode -synctex=1 -kanji=utf8 %S';

#--------------------------------------------------#
# 2. BibTeX Setting (if you use bibtex to make references)
#--------------------------------------------------#

$bibtex = 'pbibtex %O %B -kanji=utf8';

#--------------------------------------------------#
# 3. DVI-PDF Converter Setting (if you make pdf from dvi)
#--------------------------------------------------#

#$dvipdf = 'dvipdfmx %O -o %D %S';

#--------------------------------------------------#
# 4. PDF Mode Setting
#   0: don't make pdf
#   1: use pdflatex (English)
#   2: use ps2pdf
#   3: make pdf from dvi (Japanese)
#--------------------------------------------------#

$pdf_mode = 1; 

#--------------------------------------------------#
# 5. Previewer Settings
#--------------------------------------------------#

##### Use pdf-view of tex editors #####
#$pdf_previewer = 'exit';

##### If you use external previewers (you have to verify paths of pdf previewers and tex editors) #####
##### Use SumatraPDF and VS code inverse search #####
$pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance -inverse-search "\"%USERPROFILE%\AppData\Local\Programs\Microsoft VS Code\Code.exe\" -g \"%f\":\"%l\"" %O %S';

##### Use SumatraPDF and Atom inverse search #####
# $pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance -inverse-search "\"%USERPROFILE%\AppData\Local\atom\bin\atom.cmd\" \"%f:%l\"" %O %S';

#--------------------------------------------------#
# 6. Other Settings
#--------------------------------------------------#

##### Don't preserve temporary files #####
$pvc_view_file_via_temporary = 0;

#--------------------------------------------------#
# References
# * https://ichiro-maruta.blogspot.com/2016/01/atom-latex-on-windows.html
# * https://qiita.com/Rumisbern/items/d9de41823aa46d5f05a8
#--------------------------------------------------#

